Chartist: Task-driven Eye Movement Control for Chart Reading

To design data visualizations that are easy to comprehend, we need to understand how people with different interests read them. Computational models of predicting scanpaths on charts could complement empirical studies by offering estimates of user performance inexpensively; however, previous models have been limited to gaze patterns and overlooked the effects of tasks. Here, we contribute Chartist, a computational model that simulates how users move their eyes to extract information from the chart in order to perform analysis tasks, including value retrieval, filtering, and finding extremes. The novel contribution lies in a two-level hierarchical control architecture. At the high level, the model uses LLMs to comprehend the information gained so far and applies this representation to select a goal for the lower-level controllers, which, in turn, move the eyes in accordance with a sampling policy learned via reinforcement learning. The model is capable of predicting human-like task-driven scanpaths across various tasks. It can be applied in fields such as explainable AI, visualization design evaluation, and optimization. While it displays limitations in terms of generalizability and accuracy, it takes modeling in a promising direction, toward understanding human behaviors in interacting with charts.

==> Sections/3-Analysis-legacy.tex <==
\section{An Analysis of Task-driven Scanpaths on Charts}
\label{sec:analysis}


For more effective modeling, we conducted an analysis based on the human scanpaths collected in a previous work~\cite{polatsek2018exploring} to better understand task-driven scanpaths on charts. The data includes 47 users's eye movement data on visualizations when solving analytical tasks. Our analysis includes 15 statistical charts  (e.g., bar chart, line chart, and scatterplot). We excluded other types of graphs, such as maps and information graphics, as they could potentially increase the exploration rate due to the complexity of their visual representations. 
Here are the three analytical tasks in the study:

\begin{itemize}
    \item[1)] \textit{Retrieve value (RV)}: Given a specific target, find the data value of that target (e.g., \textit{what is the value of a category?});
    \item[2)] \textit{Filter (F)}: Given a concrete condition, find which data point satisfies it (e.g., \textit{which category has a specific value?});
    \item[3)] \textit{Find extreme (FE)}: Find the data point showing an extreme value of an attribute within the data set (e.g., \textit{which category has the highest/lowest value?}).
\end{itemize}


The analysis in the previous study summarizes insightful overall findings: Scanpaths for the same visualization task are more coherent than exploratory free-viewing. The task results in top-down guidance of visual attention, with bottom-up image saliency having a lesser impact on visual attention.
Beyond looking at the general analysis from the previous study, We introduce more detailed metrics to show the statistical summary of task-driven scanpaths on charts. The measurements used are inspired by \cite{goldberg2010comparing}, summarized as follows:

\begin{itemize}
    \item \textit{Number of fixations}: The length of a scanpath can be measured by the count of eye fixations separated by saccades. 
    \item \textit{Fixation on task-dependent AOI ratio}: Task-dependent AOIs are regions that are relevant to the task, such as value labels, text labels, and data points~\cite{polatsek2018exploring}. When people focus on these areas, it indicates how they are processing the task. Inspired by the metric of Hit Any AOI Rate~\cite{wang22_etvis}, this measurement provides a summary of the overall visual attention on the task-related regions.
    \item \textit{Percentage of fixations within each area}: The metric shows the percentage of time spent looking at different parts of a chart. This helps summarize where people are focusing their visual attention. We look at key areas on charts: the title, the marks (like bars or data points), and the axes. The percentages are calculated by dividing the number of fixations in a specific area by the total number of fixations.
    \item \textit{Fixation transitions}: This metric represents the average number of times the eyes move from one area to another while performing a task. It helps us understand how often the eye fixations shift between different areas. Frequent fixation transitions may indicate that there is room for improvement in the design of the chart, such as bringing related elements closer together.
    \item \textit{Revisit frequencies}: The average number of fixation returns to an area during a task.
\end{itemize}

% \begin{figure}[!t]
% \centering
%   \includegraphics[width=0.7\textwidth]{Images/analysis-scanpath.png}
%   \caption{The deep analysis of task-driven scanpaths}
%   \label{fig:analysis}
% \end{figure}

Our analysis indicates the detailed statistical summary of task-driven eye movement behaviors. 
The main findings are characterized as follows:
1) \textit{More fixations than free viewing}: We found the number of fixations in the task-driven scanpaths on charts (81.9 on average) is much larger than the number in free-viewing tasks (37.4 on average). It indicates the difficulty of the analytical tasks than the free viewing of charts.
2) \textit{A small portion of fixations on task-dependent AOIs}: Although the scanpath is task-driven, we figure out most of the eye movement is not on the task-dependent regions as the fixation on task-dependent AOI rate is only 9.1\%. It hints that people may spend more time on other stuff on the charts, like gathering information or confirmation.
3) \textit{Preference of visual attention on the axi}s: People spend most of their fixations on the axis (40.6\% on average), then the region of graphic marks (32.2\% on average). This might be because the three analytical tasks are highly related to values, not the other visual features. 
4) \textit{Frequent fixation transitions}: We identified that the number of fixation transitions is high (about 18.9 times). On average, there are about 4 continuous fixations after each fixation transition.
5) \textit{Frequent revisits}: Human data also has high revisit rates. Spatially, they revisit marks (8.7 times on average) and axis (9.0 times on average), which means users frequently double-check data information in the chart for the answer. Frequent revisits may be due to forgetting the information.
These findings help with the consideration of model design and will be valuable for evaluating the human-likeness of predicted scanpaths (see evaluation metrics in Table.~\ref{tab:benchmark}).


% \subsection{Analysis Results}
% \input{Tables/phenomena}

% The main results aggregated at the task level are summarized in Table~\ref{tab:phenomena}.
% 705 scanpaths from 47 participants, looking at 
% General scanpath length: In task-driven scanpaths on statistical charts, the average number of fixations is about 76.0 (w/ legend) and 88.4 (w/o legend). ``Find extreme'' has a slightly shorter average than the other two tasks. Without legends, the scanpath can be shortened by over 10 fixations in ``retrieve value'' and ``filter'', but it does not affect the length for ``find extreme''.


==> Sections/6-Conclusion-legacy.tex <==
\section{Discussion}

% We discuss the main findings and implications from our study, followed by the limitations and future work of our work.

In this work, we present a computational model that simulates users eye movements on charts when solving visual analytical tasks. 
The results in Table~\ref{tab:benchmark} demonstrate that the model is able to accurately simulate human-like eye movements when performing analytical tasks. The predicted scanpaths closely match the spatial positions and temporal orders of human visual scanpaths. 
In addition, the model also shows similar behaviors observed in human data, such as the sequence of task-related focal points, the distribution of fixations on different areas of the chart, and the frequency of transitions and revisits.

The model benefits from the hierarchical control architecture~\cite{eppe2022intelligent}. This architecture involves two controllers with different abilities. The high-level controller sets goals based on memory, while the low-level controller is responsible for gaze control based on pixel-level observation. Large language models are well-suited for this hierarchical architecture due to their strong reasoning abilities at the high-level control.
By following the principle of modeling computationally rational behavior models~\cite{chandramouli2024workflow, oulasvirta2022computational}, we gain the advantage of training the model in a controlled environment instead of relying on human eye movement data. This approach saves us from the costly and time-consuming process of collecting eye tracking data.
In our current setup, the reward function is fairly straightforward and objective, as the basic analytical tasks are all based on value lookup. However, there may be a need for additional design considerations for subjective tasks, such as clustering the data or identifying the outliers. This may require extra effort to incorporate visualization knowledge into the training environment, especially in the context of the reward function.


\subsection{Limitations and Future Work}

\paragraph{Generalizability}
Currently, the model was primarily developed and tested using bar charts, the most frequently used chart type in analysis.
The training stage was purely in our synthetic chart environment, where human eye movement data were not involved.
Still, the quantitative and qualitative performance of our model showcases the closet to human data.
%To clarify, our approach and all these baselines never use human eye movement data on the testing charts in the dataset. Furthermore, other than other baseline approaches relying on prior human eye movement data in other datasets as the training set, no such eye movement data is included in the training of our approach.
However, the model's architecture is designed with the flexibility to support other types of charts. By expanding the diversity of synthetic data or incorporating labeled charts, we can extend the model's chart-wise capabilities.
To prove that, we tested the model's performance on a line chart by manually labeling all potential AOIs and training it with random tasks (e.g., asking the value for a randomly selected category). The trained model shows good performance when compared to the human scanpath on the task (Fig.~\ref{fig:case}). By expanding the synthetic environment to cover a wider range of charts through visualization engineering, we can develop models that can be tailored for specific uses on other types of charts in the future.

\begin{figure}[!h]
\centering
  \includegraphics[width=0.75\textwidth]{Images/case.png}
  \caption{A case illustrates the extension of our approach to a line chart.}
  \label{fig:case}
\end{figure}

\paragraph{Chart question answering}
Beyond scanpath prediction, our model, on the other hand, can answer questions using reasoning abilities from LLMs. However, its ability to answer questions is limited to the textual information present in the chart. For example, if a bar is located between two labeled values (10 and 15), the model may provide these numbers as an answer, but not the exact answer. 
While the model's main focus is not on answering questions based on chart data, it possesses the potential to enhance question-answering accuracy by improving spatial perception capabilities.
Some existing methods specifically designed for chart question answering perform well, as mentioned in~\cite{masry2022chartqa}. These methods utilize the full visual information from the chart as input, and the most recent work has achieved an accuracy of 81.3\% accuracy~\cite{cuarbune2024chart}, demonstrating the power of integration of multi-modal large language models.

\paragraph{Application}
One potential usage application of the model is to help with the evaluation and optimization of visualization design~\cite{shin2023perceptual}. Like other design disciplines, visualization design requires user feedback for continual iterations. When visualization designers are creating charts for specific tasks, they may wonder whether the design is good enough for delivery. With the predicted scanpaths from the model, they can easily access quick and affordable feedback before a design is evaluated in an expensive real user study.

% Discussion: It should return to talk about hierarchical control (that's the main contribution)




% In this work, we present a computational model for controlling eye movements when analyzing charts. 


% Usage case: The evaluation and optimization of task-driven visualization design.

%Theoratical assumptions
% Alternative way to build them
% Applicability

% \subsection{Optimal Viewing Sequence}

% \begin{itemize}
%     \item \textbf{Retrieve value}: ``A target item label has to be searched. Then, the value label of the target data point.''
%     \item \textbf{Filter}: ``Read one or multiple item labels of targets whose attribute values fulfill the given criteria.''
%     \item \textbf{Find Extreme}: ``Users may directly search for the data point without reading value labels if data entities are sorted according to the attribute’s value in question.''
% \end{itemize}

==> Tables/ablation.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation study}
\begin{tabular}{l|lccc}
\hline \multicolumn{1}{l}{ \textbf{Task} } &  \textbf{Method} &\begin{tabular}{c} 
\textbf{Accuracy}
\end{tabular} & \begin{tabular}{c} 
\textbf{Efficiency}
\end{tabular} \\
\hline 
\multirow{2}*{Retrieve value} & Direct LLM & * & * \\
~ & Ours & * & * \\
\hline 
\multirow{2}*{Filter} & Direct LLM & * & * \\
~ & Ours & * & * \\
\hline 
\multirow{2}*{Find extreme} & Direct LLM & * & * \\
~ & Ours & * & * \\
\hline
\end{tabular}
\label{tab:ablation}
\end{table}

==> Tables/benchmark_backup.tex <==
\definecolor{bad}{rgb}{0.99608,0.87843,0.82353}
\definecolor{good}{rgb}{0.89804, 0.96078, 0.87843}

\textbf{Andreas: I suggest to move the "Ours" column forward, before "Human". makes comparing numbers between Ours and Human easier. And doesn't "hide" the most important results at the end; add thousand delimiter
}

\begin{table}[htbp]
\centering
\caption{A quantitative benchmark of the task-driven human scanpaths on bar charts. The best results are shown in {\cellcolor{good}} \textbf{bold}. For eye movement statistics, all results within 1 standard deviation from human are \underline{underlined}. All the good results are colored green.}
\begin{tabular}{cl p{15mm} p{15mm}p{15mm}p{15mm}p{15mm}}
\toprule
\textbf{Task Type} & \textbf{Metric} & \textbf{Human} & \textbf{DGiii~\cite{kummerer2022deepgaze}} & \textbf{VQA~\cite{chen2021predicting}} & \textbf{UMSS~\cite{wang2023scanpath}} & \textbf{Ours} \\
\midrule 
\multirow{15}*{\makecell[l]{Retrieve value}} 
& Sequence Score~$\uparrow$ (\textit{mean}) & 0.486 & 0.345 & 0.127 & 0.246 & {\cellcolor{good}} \textbf{0.413} \\ % & {\cellcolor{good}} \textbf{0.380}\\
& Sequence Score~$\uparrow$ (\textit{best}) & 0.638 & 0.404 & 0.151 & 0.312 & {\cellcolor{good}} \textbf{0.472} \\ %{\cellcolor{good}} \textbf{0.484}\\
& LEV~$\downarrow$ (\textit{mean}) & 154.7 & 189.7 & 164.6 & 157.4 & {\cellcolor{good}} \textbf{151.8} \\ % 188.4\\
& LEV~$\downarrow$ (\textit{best}) & 121.5 & 181.4 & 162.5 & 150.9 & {\cellcolor{good}} \textbf{141.7} \\ %153.0\\
& DTW~$\downarrow$ (\textit{mean}) & 26018 & 37160 & 36703 & {\cellcolor{good}} \textbf{26305} & 28172 \\ %34092\\
& DTW~$\downarrow$ (\textit{best}) & 17692 & 30574 & 33121 & {\cellcolor{good}} \textbf{21081} & 23541 \\ %25081\\
~ & Number of fixations        & 88.6\,(57.0) & - & 8.5\,(0.5) & 22.2\,(3.7) & {\cellcolor{good}} \textbf{48.4}\,(4.9)\\
% ~ & Saccade length             & 179.2 & 257.8 & 102.1 & 302.1 & 231.3\\
~ & Task AOIs ratio (\%)       & 10.4\,(7.8) & {\cellcolor{good}} \textbf{5.8}\,(8.2) & 1.2\,(3.9) & {\cellcolor{good}} \underline{3.8}\,(5.8) & {\cellcolor{good}} \underline{4.1}\,(4.3)\\
~ & Fixation-on-title ratio (\%)   & 10.5\,(9.3) & 33.5\,(13.4) & 2.8\,(5.7) & {\cellcolor{good}} \textbf{13.7}\,(8.7) & {\cellcolor{good}} \underline{5.3}\,(3.3)\\
~ & Fixation-on-mark ratio (\%)    & 31.5\,(13.9) & 15.3\,(10.3) & 64.0\,(24.3) & 51.1\,(12.8) & {\cellcolor{good}} \textbf{38.6}\,(21.3)\\
~ & Fixation-on-axis ratio (\%)    & 47.5\,(19.0) & {\cellcolor{good}} \underline{28.6}\,(10.5) & 23.8\,(20.8) & 21.5\,(14.7) & {\cellcolor{good}} \textbf{43.9}\,(17.2)\\
~ & Fixation transitions & 20.1\,(12.4) & 33.9\,(9.2) & 3.4\,(1.7) & {\cellcolor{good}} \underline{10.6}\,(3.3) & {\cellcolor{good}} \textbf{16.7}\,(7.0)\\
~ & Revisit frequency title    & 2.6\,(2.4) & 10.1\,(2.6) & {\cellcolor{good}} \underline{0.2}\,(0.5) & {\cellcolor{good}} \textbf{2.1}\,(1.2) & {\cellcolor{good}} \underline{2.0}\,(1.3)\\
~ & Revisit frequency mark     & 7.9\,(5.1) & {\cellcolor{good}} \textbf{8.6}\,(4.4) & 1.8\,(0.8) & {\cellcolor{good}} \underline{4.3}\,(1.5) & {\cellcolor{good}} \underline{6.8}\,(3.4)\\
~ & Revisit frequency axis     & 7.9\,(4.4) & {\cellcolor{good}} \underline{12.4}\,(3.2) & 1.3\,(1.0) & 3.0\,(1.9) & {\cellcolor{good}} \textbf{7.8}\,(3.4)\\
\midrule 
\multirow{15}*{\makecell[l]{Filter}} 
& Sequence Score~$\uparrow$ (\textit{mean}) & 0.452 & 0.321 & 0.149 & 0.271 & {\cellcolor{good}} \textbf{0.379} \\ %{\cellcolor{good}} \textbf{0.357} \\
& Sequence Score~$\uparrow$ (\textit{best}) & 0.655 & 0.382 & 0.175 & 0.340 & {\cellcolor{good}} \textbf{0.460} \\ % {\cellcolor{good}} \textbf{0.501}\\
& LEV~$\downarrow$ (\textit{mean}) & 165.8 & 201.5 & 167.6 & 161.0 & {\cellcolor{good}} \textbf{155.3} \\ %187.6\\
& LEV~$\downarrow$ (\textit{best}) & 114.5 & 192.6 & 164.7 & 153.5 & {\cellcolor{good}} \textbf{146.4} \\ %{\cellcolor{good}} \textbf{139.3}\\
& DTW~$\downarrow$ (\textit{mean}) & 23732 & 38139 & 29141 & {\cellcolor{good}} \textbf{22817} & 24617 \\ %32243\\
& DTW~$\downarrow$ (\textit{best}) & 15238 & 30981 & 25233 & {\cellcolor{good}} \textbf{17725} & 19879 \\ %23259\\
& Number of fixations & 89.1\,(68.7) & - & 8.5\,(0.5) & {\cellcolor{good}} \underline{22.2}\,(3.7) & {\cellcolor{good}} \textbf{48.7}\,(3.3)\\
% ~ & Saccade length & 163.6 & 257.8 & 102.1 & 302.1 & 230.0\\
& Task AOIs ratio (\%) & 19.1\,(14.4) & {\cellcolor{good}} \underline{5.8}\,(8.2) & {\cellcolor{good}} \underline{13.9}\,(17.4) & 3.8\,(5.8) & {\cellcolor{good}} \textbf{10.6}\,(11.2)\\
& Fixation-on-title ratio (\%) & 5.5\,(5.7) & 33.5\,(13.4) & {\cellcolor{good}} 2.0\,(5.0) & 13.7\,(8.7) & {\cellcolor{good}} \textbf{4.7}\,(2.3)\\
& Fixation-on-mark ratio (\%) & 41.9\,(18.4) & 15.3\,(10.3) & 68.8\,(23.5) & {\cellcolor{good}} \underline{51.1}\,(12.8) & {\cellcolor{good}} \textbf{49.1}\,(21.8)\\
& Fixation-on-axis ratio (\%) & 43.3\,(20.9) & {\cellcolor{good}} \underline{28.6}\,(10.5) & 20.6\,(19.4) & 21.5\,(14.7) & {\cellcolor{good}} \textbf{36.7}\,(19.4)\\
& Fixation transitions & 18.4\,(13.3) & 33.9\,(9.2) & 3.2\,(1.7) & {\cellcolor{good}} \underline{10.6}\,(3.3) & {\cellcolor{good}} \textbf{15.3}\,(5.8)\\
& Revisit frequency title & 1.4\,(1.7) & 10.1\,(2.6) & {\cellcolor{good}} \underline{0.2}\,(0.4) & {\cellcolor{good}} \underline{2.1}\,(1.2) & {\cellcolor{good}} \textbf{2.0}\,(1.1)\\
& Revisit frequency mark & 7.7\,(5.6) & {\cellcolor{good}} \textbf{8.6}\,(4.4) & 1.8\,(0.8) & {\cellcolor{good}} \underline{4.3}\,(1.5) & {\cellcolor{good}} \underline{6.0}\,(2.9)\\
& Revisit frequency axis & 8.0\,(5.5) & {\cellcolor{good}} \underline{12.4}\,(3.2) & 1.2\,(1.1) & {\cellcolor{good}} \underline{3.0}\,(1.9) & {\cellcolor{good}} \textbf{7.0}\,(2.5)\\
\midrule
\multirow{15}*{\makecell[l]{Find extrema}}
& Sequence Score~$\uparrow$ (\textit{mean}) & 0.454 & 0.362 & 0.126 & 0.253 & {\cellcolor{good}} \textbf{0.378} \\ %{\cellcolor{good}} \textbf{0.364}\\
& Sequence Score~$\uparrow$ (\textit{best}) & 0.627 & 0.428 & 0.149 & 0.320 & {\cellcolor{good}} \textbf{0.457}\\ %{\cellcolor{good}} \textbf{0.496}\\
& LEV~$\downarrow$ (\textit{mean}) & 167.3 & 188.9 & 168.3 & 160.5 & {\cellcolor{good}} \textbf{151.4} \\ %176.4\\
& LEV~$\downarrow$ (\textit{best}) & 123.9 & 180.9 & 168.3 & 155.6 & {\cellcolor{good}} \textbf{143.9} \\ % {\cellcolor{good}} \textbf{151.2}\\
& DTW~$\downarrow$ (\textit{mean}) & 27701 & 36878 & 34287 & {\cellcolor{good}} \textbf{25398} & 26677 \\ %32728\\
& DTW~$\downarrow$ (\textit{best}) & 18626 & 30400 & 31379 & {\cellcolor{good}} \textbf{20631} & 22537 \\ % 25960\\
~ & Number of fixations        & 91.9\,(64.9) & - & 8.5\,(0.5) & 22.2\,(3.7) & {\cellcolor{good}} \textbf{46.2}\,(6.8)\\
% ~ & Saccade length             & 190.8 & 257.8 & 102.1 & 302.1 & 274.9\\
~ & Task AOIs ratio (\%)       & 1.7\,(3.4) & 5.8\,(8.2) & 0\,(0) & {\cellcolor{good}} \underline{3.8}\,(5.8) & {\cellcolor{good}} \textbf{0.2}\,(0.7)\\
~ & Fixation-on-title ratio (\%) & 12.0\,(8.6) & 33.5\,(13.4) & 2.4\,(5.5) & {\cellcolor{good}} \textbf{13.7}\,(8.7) & {\cellcolor{good}} \underline{5.4}\,(3.2)\\
~ & Fixation-on-mark ratio (\%)  & 34.4\,(19.4) & {\cellcolor{good}} \underline{15.3}\,(10.3) & 64.7\,(25.6) & {\cellcolor{good}} \underline{51.1}\,(12.8) & {\cellcolor{good}} \textbf{41.6}\,(15.6)\\
~ & Fixation-on-axis ratio (\%)  & 39.7\,(22.8) & {\cellcolor{good}} \underline{28.6}\,(10.5) & {\cellcolor{good}} \underline{23.7}\,(22.9) & {\cellcolor{good}} \underline{21.5}\,(14.7) & {\cellcolor{good}} \textbf{40.7}\,(11.3)\\
~ & Fixation transitions        & 22.6\,(16.8) & {\cellcolor{good}} \underline{33.9}\,(9.2) & 3.0\,(1.6) & {\cellcolor{good}} \underline{10.6}\,(3.3) & {\cellcolor{good}} \textbf{16.0}\,(4.9)\\
~ & Revisit frequency title     & 3.2\,(3.3) & 10.1\,(2.6) & {\cellcolor{good}} \underline{0.2}\,(0.5) &{\cellcolor{good}} \textbf{2.1}\,(1.2) & {\cellcolor{good}} \underline{2.0}\,(1.1)\\
~ & Revisit frequency mark      & 8.1\,(5.6) & {\cellcolor{good}} \textbf{8.6}\,(4.4) & 1.7\,(0.8) & {\cellcolor{good}} \underline{4.3}\,(1.5) & {\cellcolor{good}} \underline{6.1}\,(2.4)\\
~ & Revisit frequency axis      & 8.9\,(5.7) & {\cellcolor{good}} \underline{12.4}\,(3.2) & 0.8\,(1.1) & 3.0\,(1.9) & {\cellcolor{good}} \textbf{7.7}\,(2.3)\\
\bottomrule
\end{tabular}
\label{tab:benchmark}
\end{table}

% ~ & ~  & ~ & 13/45 & 6/45 & 25/45 & 39/45\\
% ~ & ~  & ~ & 13/27 & 6/27 & 19/27 & 27/27\\

==> Tables/order.tex <==
\begin{table}[htbp]
\centering
\caption{Order of viewing sequence}
\begin{tabular}{l|lccc}
\hline \multicolumn{1}{l}{ Task } &  Method &\begin{tabular}{c} 
Kendall rank
\end{tabular} & \begin{tabular}{c} 
Spearman’s coefficient
\end{tabular} \\
\hline 
\multirow{2}*{Read value} & Human & * & * \\
~ & Ours & * & * \\
\hline 
\multirow{2}*{Filter} & Human & * & * \\
~ & Ours & * & * \\
\hline 
\multirow{2}*{Find extreme} & Human & * & * \\
~ & Ours & * & * \\
\hline
\end{tabular}
\label{tab:order}
\end{table}

==> Tables/phenomena.tex <==
\begin{table}[htbp]
\centering
\caption{Summary statistics of task-driven human scanpaths on statistical charts}
\begin{tabular}{lrrrrrrrrrrrr}
\toprule 
\multirow{3}*{\makecell[l]{\textbf{Metric}}} & 
\multicolumn{4}{c}{\textbf{Retrieve Value}} & \multicolumn{4}{c}{\textbf{Filter}} & \multicolumn{4}{c}{\textbf{Find Extreme}} \\
~ & \multicolumn{2}{c}{w/ L} & \multicolumn{2}{c}{w/o L} & \multicolumn{2}{c}{w/ L} & \multicolumn{2}{c}{w/o L} & \multicolumn{2}{c}{w/ L} & \multicolumn{2}{c}{w/o L} \\
~ & mean & $S D$ & mean & $S D$ & mean & $S D$ & mean & $S D$ & mean & $S D$ & mean & $S D$ \\
\midrule 
Number of fixations & 92.8 & 62.1 & 71.2 & 47.9 & 96.0 & 60.1 & 79.9 & 42.7 & 76.4 & 51.4 & 76.8 & 44.6\\
Task AOIs ratio (\%) & 11.3 & 7.7 & 12.1 & 9.0 & 11.5 & 8.4 & 16.8 & 14.0 & 1.2 & 2.3 & 1.9 & 3.8\\
Fixation-on-title ratio (\%) & 12.8 & 11.1 & 12.9 & 11.5 & 7.1 & 6.7 & 11.3 & 10.0 & 12.1 & 9.9 & 20.8 & 12.1\\
Fixation-on-mark ratio (\%) & 27.9 & 12.3 & 33.1 & 19.3 & 36.7 & 16.3 & 37.9 & 22.2 & 29.1 & 15.7 & 28.3 & 20.7\\
Fixation-on-axis ratio (\%) & 31.1 & 14.6 & 52.5 & 19.6 & 35.5 & 14.3 & 49.1 & 20.3 & 26.6 & 14.4 & 48.6 & 20.3\\
Fixation-on-legend ratio (\%) & 25.5 & 15.1 & - & - & 18.5 & 12.2 & - & - & 29.2 & 16.6 & - & -\\
Fixation transitions & 29.8 & 18.9 & 18.6 & 13.0 & 31.4 & 19.4 & 19.1 & 11.7 & 24.3 & 15.3 & 19.0 & 11.8\\
Revisit frequency title & 3.1 & 2.6 & 2.6 & 2.3 & 2.3 & 2.2 & 2.6 & 2.3 & 2.9 & 3.5 & 4.2 & 3.3\\
Revisit frequency mark & 10.4 & 6.8 & 7.8 & 5.8 & 11.9 & 7.6 & 7.9 & 5.3 & 7.9 & 5.0 & 6.8 & 5.3\\
Revisit frequency axis & 9.7 & 6.9 & 8.2 & 5.8 & 11.8 & 8.3 & 8.5 & 5.4 & 7.8 & 6.2 & 8.1 & 4.9\\
Revisit frequency legend & 6.7 & 5.5 & - & - & 5.3 & 4.0 & - & - & 5.8 & 3.5 & - & -\\
\bottomrule
\end{tabular}
\label{tab:phenomena}
\end{table}

% Saccade length & 174.9 & 36.9 & 170.9 & 41.4 & 173.6 & 38.9 & 165.4 & 46.7 & 193.0 & 45.5 & 177.2 & 44.4\\
% First fixation on AOI & 12.9 & 24.0 & 14.0 & 23.5 & 16.1 & 18.0 & 14.6 & 16.0 & 17.6 & 30.5 & 14.6 & 30.1\\

==> Tables/scanpath_benchmark.tex <==
\begin{table}[ht]
\centering
\caption{Similarity Benchmark.RV: retrieve value, F: filter, FE: find extreme.}
\begin{tabular}{llccccccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Observation Condition}} & \multirow{2}{*}{\textbf{Stimuli}} & \multicolumn{2}{c}{\textbf{Sequence Score~$\uparrow$}} & \multicolumn{2}{c}{\textbf{LEV~$\downarrow$}} & \multicolumn{2}{c}{\textbf{DTW~$\downarrow$}} \\
& & & & \textit{mean} & \textit{best} & \textit{mean} & \textit{best} & \textit{mean} & \textit{best} \\
\midrule 
\multirow{5}{*}{RV}& Human & Task-driven & Visualization & 0.418 & 0.612 & 167.7 & 118.4 & 25396 & 15685 \\
\cmidrule{2-10}
& DeepGaze iii~\cite{kummerer2022deepgaze} & Free-viewing & Natural image & 0.350 & 0.404 & 188.7 & 180.6 & 35160 & 29533 \\
& VQA Scanpath~\cite{chen2021predicting} & Task-driven & Natural image & 0.108 & 0.134 & 157.2 & 154.8 & 34421 & 31007 \\
& UMSS~\cite{wang2023scanpath} & Free-viewing & Visualization & 0.265 & 0.340 & 149.0 & 141.8 & 22569 & 18130 \\
& Ours & Task-driven & Visualization & * & * & * & * & * & *\\
\midrule 
\multirow{5}{*}{F} & Human & Task-driven & Visualization & 0.444 & 0.648 & 171.0 & 120.2 & 24137 & 15685 \\
\cmidrule{2-10}
& DeepGaze iii~\cite{kummerer2022deepgaze} & Free-viewing & Natural image & 0.348 & 0.408 & 191.5 & 183.1 & 35928 & 30241 \\
& VQA Scanpath~\cite{chen2021predicting} & Task-driven & Natural image & 0.098 & 0.117 & 165.7 & 164.2 & 35581 & 31681 \\
& UMSS~\cite{wang2023scanpath} & Free-viewing & Visualization & 0.259 & 0.330 & 157.5 & 151.5 & 22422 & 17767 \\
& Ours & Task-driven & Visualization & * & * & * & * & * & *\\
\midrule 
\multirow{5}{*}{FE}& Human & Task-driven & Visualization & 0.408 & 0.607 & 162.4 & 111.0 & 24834 & 15321 \\
\cmidrule{2-10}
&DeepGaze iii~\cite{kummerer2022deepgaze} & Free-viewing & Natural image & 0.347 & 0.403 & 183.5 & 175.9 & 33604 & 28171 \\
&VQA Scanpath~\cite{chen2021predicting} & Task-driven & Natural image & 0.118 & 0.141 & 145.2 & 143.9 & 30037 & 27098 \\
&UMSS~\cite{wang2023scanpath} & Free-viewing & Visualization & 0.282 & 0.361 & 138.5 & 132.6 & 21104 & 16865 \\
& Ours & Task-driven & Visualization & * & * & * & * & * & * \\
\bottomrule
\end{tabular}
\label{tab:scanpath_benchmark}
\end{table}


==> Tables/scanpath_benchmark_barchart.tex <==
\begin{table}[ht]
\centering
\caption{Similarity Benchmark on Bar charts (economics\_85, for finetuning only).}
\begin{tabular}{llccccccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Observation Condition}} & \multirow{2}{*}{\textbf{Stimuli}} & \multicolumn{2}{c}{\textbf{DTW~$\downarrow$}} & \multicolumn{2}{c}{\textbf{LEV~$\downarrow$}} & \multicolumn{2}{c}{\textbf{SS~$\uparrow$}}  \\
& & & & \textit{mean} & \textit{best} & \textit{mean} & \textit{best} & \textit{mean} & \textit{best} \\
\midrule 
\multirow{5}{*}{RV}& Human & Task-driven & Visualization & * & * & * & * & * & *\\
\cmidrule{2-10}
& DeepGaze iii~\cite{kummerer2022deepgaze} & Free-viewing & Natural image & 47899 & 38872 & 211 & 202 & \textbf{0.386} & 0.444\\
& VQA Scanpath~\cite{chen2021predicting} & Task-driven & Natural image & * & * & * & * & * & * \\
& UMSS~\cite{wang2023scanpath} & Free-viewing & Visualization& \textbf{39522} & \textbf{32870} & 216 & 210  & 0.201 & 0.248\\
& Ours & Task-driven & Visualization & 41988 & 34687 & \textbf{209} & \textbf{194} & 0.340 & \textbf{0.515}\\

\midrule 
\multirow{5}{*}{F} & Human & Task-driven & Visualization & * & * & * & * & * & *\\
\cmidrule{2-10}
& DeepGaze iii~\cite{kummerer2022deepgaze} & Free-viewing & Natural image & 39010 & 30359 & 167 & 158 & \textbf{0.393} & 0.460\\
& VQA Scanpath~\cite{chen2021predicting} & Task-driven & Natural image & * & * & * & * & * & * \\
& UMSS~\cite{wang2023scanpath} & Free-viewing & Visualization & \textbf{20644}  & \textbf{16051} & \textbf{124} & 118 & 0.279 & 0.344\\
& Ours & Task-driven & Visualization & 21730 & 16453 & \textbf{124} & \textbf{113} & 0.299 & \textbf{0.567}\\
\midrule 
\multirow{5}{*}{FE}& Human & Task-driven & Visualization & * & * & * & * & * & *\\
\cmidrule{2-10}
&DeepGaze iii~\cite{kummerer2022deepgaze} & Free-viewing & Natural image & 41641 & 33964 & 185 & 175 & \textbf{0.437} & 0.503\\
&VQA Scanpath~\cite{chen2021predicting} & Task-driven & Natural image & * & * & * & * & * & * \\
&UMSS~\cite{wang2023scanpath} & Free-viewing & Visualization & 31697 & \textbf{25447} & 176 & 169 & 0.225 & 0.274\\
& Ours & Task-driven & Visualization & \textbf{31262} & 25650 & \textbf{172} & \textbf{159} & 0.259 & \textbf{0.521} \\
\bottomrule
\end{tabular}
\label{tab:scanpath_benchmark_barchart}
\end{table}

